MAPO: A Multi-Objective Model for IoT Application Placement in a Fog Environment

The emergence of the Fog computing paradigm that leverages in-network virtualized resources raises important challenges in terms of resource and IoT application management in a heterogeneous environment offering only limited computing resources. In this work, we propose a novel Pareto-based approach for application placement close to the data sources called Multiobjective IoT application Placement in fOg (MAPO). MAPO models applications based on a finite state machine and uses three conflicting optimization objectives, namely completion time, energy consumption, and economic cost, considering both the computation and communication aspects. In contrast to existing solutions that optimize a single objective value, MAPO enables multi-objective energy and cost-aware application placement. To evaluate the quality of the MAPO placements, we created both simulated and real-world testbeds tailored for a set of medical IoT application case studies. Compared to the state-of-the-art approaches, MAPO reduces the economic cost by up to 27%, while decreasing the energy requirements by 23-68%, and optimizes the completion time by up to 7.3 times.

==> artifact.tex <==
%\textbf{Reproducibility artifact}\par
%We run 6 experiments comparing MAPO with FSPP, and EW. We model two component based applications in terms of number of CPU instructions, memory, storage and bandwidth that they require.

%For real-world testbed, we exploit four Raspberry pi devices as the Edge devices and one Lenovo personal computer as CDC. 
%We installed SysBench \cite{kopytov2017sysbench} through the system package manager on the containerized devices. We utilize SysBench to emulate the execution of application components with stressing the CPU and MEM by calculating the prime numbers in the set of MaxPrime=$\{400,800,1500,3000\}$. While executing this command in a single loop with a limit of one thousand, we calculate the amount of CPU utilization with Linux \texttt{top} command.
%We emulate the data transferred between application components by generating and sending data-files with various sizes. Every device just runs one container to execute the components assigned to it.
%For the fixed CPU workload scenario evaluation, we investigate the mental health care components, shown in Section~\ref{MHC}, with different CPU processing speed requirements that we respectively set to $\{256,512,256,1024,2048,256,256\}$ MI.
